Better Software Analytics via "DUO": Data Mining Algorithms Using/Used-by Optimizers

This paper claims that a new field of empirical software engineering research and practice is emerging: data mining using/used-by optimizers for empirical studies or DUO. For example, data miners can generate models that are explored by optimizers. Also, optimizers can advise how to best adjust the control parameters of a data miner. This combined approach acts like an agent leaning over the shoulder of an analyst that advises "ask this question next" or "ignore that problem, it is not relevant to your goals". Further, those agents can help us build "better" predictive models, where "better" can be either greater predictive accuracy or faster modeling time (which, in turn, enables the exploration of a wider range of options). We also caution that the era of papers that just use data miners is coming to an end. Results obtained from an unoptimized data miner can be quickly refuted, just by applying an optimizer to produce a different (and better performing) model. Our conclusion, hence, is that for software analytics it is possible, useful and necessary to combine data mining and optimization using DUO.

==> fig6timeline.tex <==
\begin{table}[!htbp]
{\small
\begin{tabular}{|p{.99\linewidth}|}\hline
{\scriptsize  
\begin{tabular}{rrl}
2006 & 4\% & \rule{4mm}{2mm}\\
2007 & 4\% &\rule{4mm}{2mm}\\
2008 & 7\% & \rule{7mm}{2mm}\\
2010 & 11\% & \rule{11mm}{2mm}\\
2011 & 4\% & \rule{4mm}{2mm}\\
2012 & 7\% & \rule{7mm}{2mm}\\
2013 & 11\% & \rule{11mm}{2mm}\\
2015 & 4\% & \rule{4mm}{2mm}\\
2016 & 7\% & \rule{7mm}{2mm}\\
2017 & 7\% & \rule{7mm}{2mm}\\
2018 & 34\% & \rule{34mm}{2mm}\\
\end{tabular}
}\\\hline
\end{tabular}}
\caption{Papers in our literature review according to years.}\label{tbl:timeline}
\end{table}

==> old/claim1.tex <==
\section{Claim1: Optimization and data mining are very similar}\label{sec:claim1}

At first glance, the obvious connection between data miners and optimizers is that the former build models from data while the latter can be used to exercise those models (in order to find good choices within a model). % to find ``best'' regions (where ``best'' is defined according to some user-specific goals).  That is, optimizers can be used to refine the insights gained from data mining. <--- I don't think that readers will be able to understand this at this point yet. So, I've deleted it and replaced it.
%
However, a much more profound connection between data mining and optimization can be seen if we look ``under the hood'' to reflect on the core semantics of these supposedly separate kinds of algorithms.
In order to explain this, we need to formally define optimization and data mining problems. %Understanding such definitions requires basic knowledge of algebra. 
%To facilitate understanding, this section will be explained by considering a specific class of data mining problems which can be solved through supervised learning. However, the notions explained hereby can be extended or adapted to other data mining problems.

Without loss of generality, an optimization problem is of the following format~\cite{OptDef}:
\begin{equation}
\begin{tabular}{ll}
minimize        & $f_i(\textbf{a})$, $i=1,2,\cdots,n$ \\
subject to      & $g'_j(\textbf{a}) \leq 0$, $j=1,2,\cdots,n'$ \\
                & $g''_k(\textbf{a}) = 0$, $k=1,2,\cdots,n''$ \\
\end{tabular}
\label{eq:optimization-problem}
\end{equation}

%\vspace{3mm}
\noindent where $\textbf{a} = (a_1,\cdots, a_m) \in \textbf{A}$ is the optimization variable of the problem\footnote{The optimization variable is usually identified by the symbol $\textbf{x}$. However, we use the symbol $\textbf{a}$ here to avoid confusion with the terminology used by data mining, which is introduced later in this section.}, $f_i(\textbf{a}): \textbf{A} \rightarrow {\rm I\!R}$ are the objective functions (goals) to be minimized, $g'_j(\textbf{a})$ are inequality constraints, and $g''_k(\textbf{a})$ are equality constraints. Sometimes, there are no constraints (so $n'=0$ and $n''=0$). Also, we say a {\em multi-objective problem} has $n>1$ objectives, as opposed to a {\em single-objective problem}, where $n=1$.

One obvious question about this general definition is ``where do the functions $f,g',g''$ come from?''. Traditionally, these have been built by hand but,
as we shall see below, $f,g',g''$ can be learned via data mining. That is, optimizers can {\em explore}
the functions {\em proposed} by a learner.


\input{fig3optimizers.tex}

An example of an optimization problem in the area of software engineering is to find a subset $\textbf{a}$ of requirements that maximizes value $f(\textbf{a})$ if implemented\footnote{Any maximization problem can be re-written as a minimization problem.}, given a constrained budget $g'_0(\textbf{a}) \leq 0$, where $g'_0(\textbf{a}) = cost(\textbf{a}) - budget$ \cite{Sagrado2011}.
Many different algorithms exist to search for solutions to optimization problems. Table \ref{tbl:optimizers} shows the optimization algorithms that have been used by the software engineering community when applying DUO.

Data mining is a problem that involves finding an approximation $\hat{h}(\textbf{x})$ of a function of the following format:
\begin{equation}\textbf{y}=h(\textbf{x})\label{eq:learning}\end{equation} 

\noindent where $\textbf{x} =(x_1,\cdots, x_p) \in \textbf{X}$ are the input variables, $\textbf{y} = (y_1,\cdots, y_q) \in \textbf{Y}$ are the output variables of the function $h(\textbf{x}): \textbf{X} \rightarrow \textbf{Y}$, \textbf{X} is the input space and \textbf{Y} is the output space. The input variables $\textbf{x}$ are frequently referred to as the independent variables or input features, whereas $\textbf{y}$ are referred to as the dependent variables or output features.  %Table \ref{tbl:learn} shows some examples that have been used in software engineering when applying DUO.

\input{fig5learners}
An example of a data mining problem in software engineering is software defect prediction~\cite{hall2012systematic}. Here, the input features could be a software component's size and complexity, and the output feature could be a label identifying the component as defective or non-defective. Many different machine learning algorithms can be used for data mining.
\tbl{learn} shows data mining  algorithms  used by the software engineering community when applying DUO.

The functions $h(\textbf{x})$ and $\hat{h}(\textbf{x})$ do \textit{not} necessarily correspond to the optimization functions $f_i(\textbf{a})$ depicted in Eq.~\ref{eq:optimization-problem}. However, the true function $h(\textbf{x})$ is unknown. Therefore, data mining frequently relies on machine learning algorithms to learn an approximation $\hat{h}(\textbf{x})$ based on a set $D = \{(x_i,y_i)\}_{i=1}^{|D|}$ of known examples (data points) from $h(\textbf{x})$. And, learning this approximation typically consists of searching for a function $\hat{h}(\textbf{x})$ that minimizes the error (or other predictive performance metrics) on examples from $D$. Therefore, learning such approximation \textit{is} an optimization problem of the following format:
\begin{equation}
\begin{tabular}{ll}
minimize        & $f_i(\textbf{a})$, $i=1,\cdots,n$ \\
\end{tabular}
\label{eq:learning-problem}
\end{equation}

\noindent where $\textbf{a} = (\hat{h}(\textbf{x}), D)$, and $f_i$ are the predictive performance metrics obtained by $\hat{h}(\textbf{x})$ on $D$. The functions $f_i(\textbf{a})$ depicted in Eq.~\ref{eq:learning-problem} thus correspond to the functions $f_i(\textbf{a})$ depicted in Eq.~\ref{eq:optimization-problem}. An example of performance metric function would be the mean squared error, defined as follows:
\begin{equation}
f(\hat{h}(\textbf{x}), D) = \frac{1}{|D|} \sum_{(x_i,y_i) \in D} (y_i -  \hat{h}(x_i))^2
\label{eq:mae}
\end{equation}

As we can see from the above, solving a data mining problem means solving an optimization problem, i.e., optimization and data mining are very similar. Indeed, several popular machine learning algorithms \textit{are} optimization algorithms. For example, gradient descent for training artificial neural networks, quadratic programming for training support vectors machines and least squares for training linear regression are optimization algorithms.

From the above, we can already see that optimization is of interest to data mining researchers, even though this connection between the two fields is not always made explicit in software engineering research. More explicit examples of how optimization is relevant to data mining in software engineering include the use of optimization algorithms to tune the parameters of the data mining algorithms, as mentioned in the beginning of this section and further explained in Sections  \ref{sec:claim3} and \ref{sec:claim5}. We consider such more explicitly posed connections between data mining and optimization as a form of DUO.

%Even   learner is trying to achieve some non-numeric goal (e.g. a binary classifier), \todo{incomplete sentence, or even$\rightarrow$every} --> I don't know who inserted this sentence here. So, I'm not sure what their intention was.

A typical distinction made between the optimization and data mining fields is data mining's need for generalization. Despite the fact that data mining uses machine learning to search for approximations $\hat{h}(\textbf{x})$ that minimize the error on a given dataset $D$, the true intention behind data mining is to search for approximations $\hat{h}(\textbf{x})$ that minimize the error on unseen data $D'$ from $h(\textbf{x})$, i.e., being able to generalize. As $D'$ is unavailable for learning, data mining has to rely on a given known data set $D$ to find a good approximation $\hat{h}(\textbf{x})$. Several strategies can be adopted by machine learning to avoid poor generalization despite the unavailability of $D'$. For instance, the performance metric functions $f_i(\hat{h}(\textbf{x}), D)$ may use regularization terms \cite{Bishop}, which encourage the parameters that compose $\hat{h}(\textbf{x})$ to adopt small values, making $\hat{h}(\textbf{x})$ less complex and thus generalize better. Another strategy is early stopping \cite{Bishop}, where the learning process stops early, before finding an optimal solution that minimizes the error on the whole set $D$. 

%This key difference can be used to further refine DUO's definition. So far, we considered DUO as the combination of data mining and optimization. We can now further refine this to say that DUO combines data mining algorithms (which learn from data and care about generalization) with optimization algorithms (which do not learn from data and do not care about generalization). 

However, even the distinction above starts to become blurry when considering that generalization can also frequently be of interest to optimization researchers. %For example, those focusing on paradigms and on methodology are quite interested in general findings.
%Several software engineering problems are both optimization and data mining problems at the same time, further highlighting the similarity between the two fields. 
For example, in software configuration optimization (Section  \ref{sec:claim4}), the true optimization functions $f_i(\textbf{a})$ are often too expensive to compute, requiring machine learning algorithms to learn approximations of such functions. Optimization functions approximated by machine learning algorithms are referred to as surrogate models, and correspond to the approximation $\hat{h}(\textbf{x})$ of Eq.~\ref{eq:learning-problem}. These approximation functions are then the one optimized, rather than the true underlying optimization function. Even though an optimization algorithm to solve this problem does not attempt to generalize, a data mining technique can do so on its behalf. We consider this as another form of DUO. %Other examples include problems problems such as ..., whose underlying optimization space is so large and complex that it requires data mining to help finding good solutions more quickly. 
Sections \ref{sec:claim3} and \ref{sec:claim4} explain how several other examples of software engineering problems are indeed both optimization and data mining problems at the same time, and how different forms of DUO can help solving these problems.

Overall, this section shows that optimization and data mining are very similar to each other, and that the typical distinction made between them can become very blurry when considering real world problems. Several software engineering problems require both optimization and generalization at the same time. Therefore, many of the ideas independently developed by the field of optimization are applicable to improve the field of data mining, and vice-versa. Sections \ref{sec:claim3} to \ref{sec:claim5} explain how useful DUO can and could be.


\iffalse
all about learning a mapping $Y=F(X)$ that connects inputs to outputs:
\bi
\item $X$ is the set $x_1, x_2, x_3...$
of {\em inputs}, also known as {\em independent variables}.
In software engineering, these might be process, product, or personnel metrics about a software project.
\item $Y$ is the set $y_1, y_2, y_3...$
of {\em outputs}, also known as {\em dependent  variables}
or {\em goals} or {\em
objectives}.
In software engineering, these might be software project
quality indicators such as project development time,
number of expected bugs, etc.
\item
In simple classification/regression problems, $Y$ has only one variable $y_1$ 
called the {\em class} that is 
discrete/numeric (respectively). 
\item
In multi-objective  problems, $Y$ can be many variables each of which we might care to minimize or maximize. 
Sometimes there is no way to satisfy all objectives, e.g., 
reduce bugs, spend less money, and deliver the project sooner.
In that case, the optimizer must learn the shape of the $Y$
so it understand the trade-offs between  objectives.
\ei

sometimes $F$ is available at the start of the inference and our job is to update $F$ (e.g. Bayes nets or stream mining)

Conversely, sometimes $F$ is missing  so the best we can do is cluster all the $X$ values of run
association rule learning over the $X$ and $Y$ values to find what sets of attribute ranges
are associated with each other. 

Further, sometimes $F$ is implicit (e.g. case based reasoning) or explicit (e.g. decision trees).

Two questions that might be asked at $Y=F(X)$ are ``what is?'' and
``what to do?'':
\bi
\item
Traditionally, the first question is explored by data miners that {\em dig} around the data looking for some buried structures.
\item
Traditionally, the second question (``what to do?'') is explored by optimizers that {\em jump} along promising trends. When such jumps land in a region that is currently under-sampled, optimizers t run $F$ some more to gather more data about that region.
\ei
In both data mining and optimization,
when $F$ is available, it can be used to assess if some guess for $X$ achieves the desired $Y$ values.
Some $F$ functions are very expensive to run (e.g. if $F$ requires synthesizing some physical object and
testing its properties; or if $F$ means ``go away and try to find a human expert that can comment on that'').
For this reason, in the data mining and optimization literature there is much interest is {\em active learning}. Active learners reflect on the models seen so far to find the most informative next question.
The total number of evaluations of $F$ can hence be minimized by only evaluating the seemingly most
informative $X$ values.
\fi

==> old/claim2.tex <==
\section{Claim2: Pragmatically, optimization and data mining are very similar}\label{sec:claim2}

As seen in  some of the examples presented in the Claim 1, we can deduce Optimization and Data miners are very similar. Now the question is do we have any examples which can pragmatically say that. Two very simple introductory examples where optimizers can help data miners and vice versa are:
\bi 
\item An optimizer can help data miner achieve massive performance improvements. For e.g., Agrawal et al. in their paper "Is Better Data better than better Data Miners"~\cite{54agrawal2018better} used DE~\cite{storn1997differential} (an optimizer) to automatically tune the parameters of SMOTE~\cite{chawla2002smote}. They observed heavy improvements in AUC and recall by 60\% and 20\% respectively. 

\item Similarly you can use a data miner to help optimizer. For e.g., Majumder et al.~\cite{88majumder2018500+} showed that by building local clusters using KMeans on the data and then running an optimizer (DE) on those local clusters can provide similar performance as Deep Learning model but 500+ times faster.
\ei

If we consider the second example, we will see that Data Miner optimizes Optimizer for runtime and then that optimizer optimizes the learner for performance. Here, optimization and data mining are very similar. 

==> old/claim3.tex <==
\section{Claim2: Optimizers can greatly improve data miners}\label{sec:claim3}
%\url{https://github.com/ai-se/dataDriveSBSE/issues/8}
%This is the most common use of {\IT}. see our lit review 
%Id2: 1, 2, 13, 26, 30,31, 35, 38,40, 42, 43, 44, 54, 55, 57, 60, 64, 88, 90, 92(dupe), 93, 94, 95(dupe),96,97,102slow
  



One of the most frequent ways to integrate
data mining and optimization is via {\em hyperparameter optimization}. This is the art of tuning the parameters that control the choices within a data miner.
While these can be set  manually\footnote{Using a process called ``engineering judgement''; i.e. guessing.} we found that several papers
in our   literature review used optimizers to
 automatically find the best parameters~\cite{54agrawal2018better,%
35fu2016,%
44liu2010evolutionary,%
97sarro2012further,%
%47tantithamthavorn2016automated,%
14zhong2004,%
102treude2018per,
42oliveira2010ga}. 
There are many reasons why this is so:

\bi
\item  These control parameters are many and varied. %and include (e.g.) the number of decision trees in a random forest. 
Even supposedly simple algorithms come with a daunting number of options. For example, the scitkit-learn toolkit lists over a dozen configuration options for Logistic Regression\footnote{
\url{https://scikit-learn.org/stable/modules/generated/sklearn.linear_model.LogisticRegressionCV.html}, accessed 30 November 2018.}. This is an important point since recent research shows that the
{\em more} settings we add to software, the {\em harder} it becomes for humans to use that software~\cite{Xu:2015}.
\item Manually fine-tuning these parameters to obtain best results for a new data set, is not only tedious, but also can be biased by a human's (mis-)understanding of the inner workings of the data miner.
%however, an automated approach to algorithm tuning is enabled by the observation that even basic heuristics do an acceptable job of improving performance over the default parameters, 
\item The hurdle to implement or apply a ``successful'' heuristic for automated algorithm tuning is low since (a) the default settings are often not optimal for the situation at hand, and (b) a large number of optimization packages are readily available~\cite{rainville2012deap,Durillo2011}.
Some data mining tools now  come 
with built-in optimizers or tuners; e.g the SMAC implementation built into
the latest versions of Weka~\cite{hutter2011sequential,Hall:2009};
or the CARET package in ``R''~\cite{JSSv028i05}.
\item
Several results report spectacular improvements 
in the performance of data miners after tuning~\cite{54agrawal2018better,%
35fu2016,%
44liu2010evolutionary,%
97sarro2012further,%
47tantithamthavorn2016automated,%
14zhong2004,%
102treude2018per}.
\ei
As evidence to the last point, we offer two examples.
Tantithamthavorn et al.~\cite{47tantithamthavorn2016automated}
applied the CARET  grid search~\cite{JSSv028i05} to improve the predictive performance of classifiers. Grid search is an exhaustive search %\footnote{Due to the exhaustive search procedure used by grid search, we do not consider it as an optimization algorithm used by {\IT} approaches. However, it can be used to illustrate the potential benefits of hyperparameter tuning.} 
across  on a pre-defined set of hyperparameter values. It is implemented as a set of for-loops, one for each hyperparameter. Inside the inner-most for-loop,
some learner is applied to some data to assess
the merits of a particular set of hyperparameters.  
Based on statistical methods, Tantithamthavorn et al. ranked all the learners in their study to find the top-ranked tuned learner. As shown in  \fig{tanit},
there is some variability in the likelihood of being top-ranked
(since their analysis was repeated for multiple runs).

\begin{figure}
\includegraphics[width=4.8in]{fig/tantit.png}
\caption{Effects of hyperparameter optimization on control parameters of  a learner from~\cite{47tantithamthavorn2016automated}. Blue dots and red triangle show the mean performance before and after tuning (respectively). 
X-axis shows different learners. Y-axis shows the frequency at which a learner was selected to be ``top-ranked'' (by a statistical analysis). Vertical lines show the variance of that selection process over repeated runs.}\label{fig:tanit}
\end{figure}
\begin{figure}
\includegraphics[width=2.4in]{fig/aucRecall.png}\includegraphics[width=2.4in]{fig/prefa.png}
\caption{Effects of hyperparameter optimization on control parameters of a data pre-processor from~\cite{54agrawal2018better}. Different colored vertical bars refer to different learners:
KNN=nearest neighbor; SVM= support vector machine; NB=naive bayes; RF=random forest; LR=logistic regression; DT=decision trees. 
X-axis shows different datasets. Y-axis   shows
the {\em after - before} values of four different performance scores: recall, precision, false alarm and AUC (area under the false positive vs true positive rate). For false alarms,
{\em better} deltas are {\em smaller}. For all other measures, the {\em larger} the {\em better}.}\label{fig:aucRecall}
\end{figure}
\noindent From \fig{tanit} we can see that:
\bi
\item Hyperparameter optimization {\em never makes performance worse}.
 We say this since the red triangles (tuned results) are never lower than their blue dot counterpart (untuned results). 
 \item
 Hyperparameter  optimization is {\em associated with some spectacular performance improvements}. Consider the first six left-hand-side blue dots at $Y=0$. These
 show  all untuned learners that are never   top-ranked. After tuning, however, the ranking of these learners is very different. Note once we tune two of these seemingly ``bad''
learners (C5.0 and AVNNet), they become part of the top three best learners.
\ei
For another example of the benefits of hyperparameter optimization, consider 
\fig{aucRecall}. This work shown by Agrawal et al.~\cite{54agrawal2018better} where differential evolution  tuned a data pre-processor called SMOTE~\cite{chawla2002smote}. SMOTE rebalances training data by discarding items of the majority class and synthesizing artificial members of the minority class. As discussed in Table~\ref{tbl:optimizers}, differential evolution~\cite{Storn:1997} is an evolutionary algorithm that uses a unique mutator that builds new candidates by combining
together three older candidates.
From \fig{aucRecall}  we can observe the same patterns seen in \fig{tanit}:
\bi
\item
 Hyperparameter optimization {\em rarely makes performance much worse}. There are some losses in precision and false alarms grow slightly. But overall, these changes are very small.
 \item
 Hyperparameter optimization is {\em associated with some spectacular performance improvements}.
 The improvements in recall can be large and the improvements in AUC are the largest
 we have ever seen of any method, ever, in the software analytics literature.
\ei

 
%Liu, Khoshgoftaar, and Seliya~\cite{44liu2010evolutionary} : here the GP becomes the learner

%temporary insertion of fig4eval.tex, to make sure it compiles
\input{fig4eval.tex}
%\url{https://github.com/ai-se/dataDriveSBSE/issues/14} 

 


% transition to next section
%In summary, hyperparameter optimization is associated with some spectacular improvements in predictor performance. However, using optimizers in this way (to tune the control parameters of a learner) can be very resource intensive. In the next section, we discuss ways that {\IT} can significantly reduce that cost by using data miners to divide and conquer complex optimization problems.
 
Another advantage of hyperparameter optimizers is that it can tune learners such that they succeed on multiple criteria. Standard learners have their goals ``hard-wired'' (e.g. minimize entropy).  This can be a useful design choice since it allows algorithm designers to produce very fast systems that scale to very large data sets.  That said, there are many   situations where the business users have {\em multiple} competing goals; e.g. deliver {\em more} functionality,
in {\em less} time, with {\em fewer} bugs. 
For further examples of multiple business goals in software analytics, see Table 23.2 of~\cite{menzies2013data}.



While the goals of data miners are often hard-wired, optimizers
can accept multiple goals as part of the specification of a problem (see the $g$ terms within Equation~\ref{eq:optimization-problem}).
This means optimizers can explore a broader range of goals than data miners. For example: 
\bi
\item
 Minku and Yao \cite{MinkuYao2013} used multi-objective evolutionary algorithms to generate neural networks for software effort estimation, with the objectives of minimizing different error metrics.
 \item
 Sarro et al.~\cite{40sarro2016} used multi-objective genetic programming for software effort estimation, with the objectives of minimizing the error and maximizing the confidence on the estimates.
\ei
 An interesting variant of the above is optimization (in the form of reinforcement learning)  is model selection over time \cite{MinkuYao2014,MinkuYao2017}. Depending on the problem being tackled, the best predictive model to be used for a given problem may change over time, due to changes suffered by the underlying data generating process of this problem. For such problems, model choice has to be continuously performed over time, rather than performed only once, prior to model usage. To deal with that in the context of software effort estimation, Minku and Yao \cite{MinkuYao2014,MinkuYao2017} monitor the predictive performance of software effort estimation models created using software effort data from different companies over time. This predictive performance was monitored based on a time-decayed performance metric derived from the reinforcement learning literature, computed over their effort estimations provided for a given company of interest over time. The models whose predictive performance are recently the best are then selected to be emphasized when performing software effort estimations to the company of interest. When combined with transfer learning \cite{MinkuYao2014}, this strategy enabled a reduction of 90\% in the number of within-company effort data required to perform software effort estimation, while maintaining or sometimes even slightly improving predictive performance. This is a significant achievement, given that the cost of collecting within-company effort data is typically very high.

\subsection{Problems with Hyperparameter Optimization}
In summary, optimization is associated with some spectacular improvements in data mining. Also,   by applying
optimizers to data miners, they can better address the  domain-specific and  goal-specific queries
of different users.

One pragmatic drawback with hyperparameter optimization is its    associated
runtime. Each time a new hyperparameter setting is evaluated, a learner must be called on some training data, then tested on some separate ``hold-out'' data. This must be repeated, many times. In practice, this can take
a long time to terminate:
\bi
\item
When replicating 
the  Tantithamthavorn et al.~\cite{47tantithamthavorn2016automated}  experiment, Fu et al.~\cite{fu2016differential}
implemented tuning using grid search and differential evolution. 
That study used   20 repeats for tuning random forests (as the target learner), and optimized four different measures
of AUC, recall, precision, false alarm, that grid search required 109 days of CPU.
Differential evolution and grid search required $10^4$ and $10^7$ seconds to terminate,
respectively\footnote{Total time to process  20 repeated runs across multiple subsets of the data, for multiple data sets.}.
\item   Xia et al.~\cite{Xia2018HyperparameterOF} reports experiments with hyperparameter optimization for software effort estimation. In their domain, depending on what data set was processed, it took
 140 to 700 minutes  (median to maximum) to compare seven ways to optimize two data miners. If that experiment is repeated 30 times for statistical validity, then the full experiment would take 70 to 340 hours (median to max).

\ei
While the above runtimes might seem practical to some researchers,
we note that other hyperparameter optimization tasks take a very long time to terminate.  Here are the two worst (i.e. slowest) examples
that we know of, seen in the recent SE literature:
\bi
\item E.g.    decades of CPU time were needed by Treude et al.~\cite{102treude2018per} to achieve a 12\% improvement over the default settings;
\item E.g.   15 years of CPU were needed in the hyperparameter optimization of software clone detectors by Wang et al.~\cite{wang2013searching}.
\ei
One way to address these slow runtimes is via (say) cloud-based CPU farms.  Cross-validation experiments can be easily parallelized just by running  each cross-val on a separate core. But 
the cumulative costs of that approach can be large.  For example, recently while developing a half million US dollar research proposal, we guesstimated how much it would cost to run the same kind of hardware as seen in related work. For that three year project,  two graduate students could easily use  \$100,000 in CPU time -- which is a large percentage of the grant (especially since, after university extracts its overhead change, that \$500K grant would effectively be \$250K).

Since using optimizers for hyperparameter optimization can be very resource intensive, the  next section discusses {\IT} to significantly reduce that cost.


==> old/claim4.tex <==
\section{Claim3: Data miners can greatly improve optimization}\label{sec:claim4}

%  This section offers some case studies
%  support {\bf Claim1} of this paper (that there is no essential difference between data miner and optimizers). In two of the   examples 
%  of this section (the work of Nair, Chen et al.~\cite{31chen2018,89chen2018sampling,87nair2017using}), there is no separate optimization module because the data miner acted as the optimizer. That is, sometimes, {\em data mining can replace, rather then merely augment, an optimizer}. 
  
The previous section mentions the benefits of optimizers for data mining, but warned that such optimization can be  slow. One way to speed up  optimization  is to divide the total problem into many small sub-problems. As discussed in this section, this can be done using data mining. That is, data mining can be used to optimize optimizers. 

Another benefit of data mining is that, as discussed below, it can generalize and summarize the results of optimization. That is, data mining can make optimization results more comprehensible.

\subsection{Faster Optimization}

It can be a very simple matter to implement data miners improving optimizers. Consider, for example,     Majumder et al.~\cite{88majumder2018500+} who were looking for the connections between posts to StackOverflow (which is a popular on-line question and answer forum for programmers):

\bi
\item
An existing deep learning approach~\cite{xu16} to that problem was so slow that it was hard to reproduce prior results. 
\item
Majumder et al. found that they could get equivalent results 500 to 900 times faster (using one core or eight cores working in parallel) just by applying k-means clustering to the data, then running their  hyperparameter optimizer (differential evolution) within each cluster.
\ei
Another example of data mining significantly improving optimization, consider the  {\em sampling} methods of Chen et al.~\cite{31chen2018,89chen2018sampling}. This team explored optimizers for a variety of (a)~software process models as well as the task of (b)~extracting products from a product line description. These are multi-objective problems that struggle to find solutions that (e.g.) minimize development cost while maximizing the delivered functionality (and several other goals as well). The product extracting task was particularly difficult. Product lines were expressed as trees of options with ``cross-tree constraints'' between sub-trees. These constraints mean that decisions in one sub-tree have to be carefully considered, given their potential effects on decisions in other sub-trees. Formally, this makes the problem NP-hard and in practice, this product extraction process was known to defeat state-of-the-art theorem provers~\cite{pohl11}, particularly for large product line models (e.g. the ``LVAT'' product line model of a LINUX kernel contained 6888 variables within a network of 343,944 constraints~\cite{89chen2018sampling}).

Chen et al. tackled this optimization problem using data mining to ``sample'' a small subset of the most informative examples. Specifically, they used
a recursive bi-clustering algorithm over a large initial population to isolate the superior candidates.
As shown in the following list, this sampling approach is somewhat different to the more standard
genetic algorithms approach:

\bi
\item Genetic algorithms (in SE) often start with an population of $N=10^2$ individuals. 
\item On the other hand, samplers start with a much larger population of $N=10^4$ individuals.
\item Genetic algorithms run for multiple {\em generations} where useful variations of individuals in generation $i$ are used to seed generation $i+1$. 
\item On the other hand, samplers run for a single generation, then terminate.
\item Genetic algorithms evaluate all $N$ individuals in all generations.
\item On the other hand, the samplers of Chen et al. evaluate pairs of distant points. If one point proves to be inferior then it is pruned along with all individuals in that half of the data. Samplers then recursively prune the surviving half. In this way, samplers only evaluate $O(2{\log}_2N)$ of the population,
\ei
Regardless of the above differences, the goal of genetic algorithms and samplers is the same:  find options that best optimize some competing set of goals. In comparisons with NSGA-II (a widely used genetic algorithm~\cite{deb02}), Chen et al.'s sampler usually optimized the same, or better, as the genetic approach. Further, since samplers only evaluate $O(2{\log}_2N)$ individuals, sampling's median cost was just 3\% of runtimes and 1\% of the number of model evaluations (compared to only running the genetic optimizer)~\cite{89chen2018sampling}.

For another example of data miners speeding up optimizers, see the work of Nair et al.~\cite{87nair2017using}. That work characterized the software configuration optimization problem as ranking a (very large) space of configuration options, without having to run tests on all those options. For example, such configuration optimizers might find a parameter setting to SQLite's configuration files that maximized query throughput. Testing each configuration requires re-compiling the whole system, then re-running the entire test suite. Hence, testing the three million valid configurations for SQLite is an impractically long process.

The key to quickly exploring such a large space of options, is  {\em surrogate modeling}; i.e. learning an approximation to the response variable being studied. The two most important properties of such surrogates are that they are much faster to evaluate than the actual model, and that the evaluations are precise. Once this approximation is available then configurations can be ranked by generating guesstimates from the surrogates. Nair et al. built their surrogates using a data miner; specifically, a regression tree learner called CART~\cite{breiman84}. An initial tree is built using a few randomly selected configurations. Then, while the error in the tree's predictions decreases, a few more examples are selected (at random) and evaluated. Nair et al. report that this scheme can build an adequate surrogate for SQLlite after 30-40 evaluated examples. 

For this paper, the key point of the Nair et al. work is that this data mining approach scales to much larger problems then what can be handled via standard optimization technology. For example, the prior state-of-the-art result in this area was work by Zuluga et al.~\cite{Zuluaga:2013} who used a Gaussian process model (GPM) to build their surrogate. GPMs have the advantage that they can be queried to find the regions of maximum variance (which can be an insightful region within which to make the next query). However, GPMs have the disadvantage that they do not scale to large models. Nair et al. found that the data mining approach scaled to models orders of magnitude larger than the more standard optimization approach of Zuluga et al. 


\subsection{Better Comprehension of User Goals}

%  For example, while exploring the multi-objectives of the requirements of London ambulances
%  Veerappa et al.~\cite{Veerappa11}. They found that when they optimized the requirements of the London Ambulance system, the result was a {\em frontier} of    hundreds of solutions like that shown in \fig{veer}. Each member of that frontier is   trying to push out on all objectives (and  perhaps failing on some). Mathematically, this is called the {\em Pareto frontier~\cite{pareto1906manuale}}. 

Aside from speeding up optimization, there are other benefits of adding data miners to optimizers. 
If we combine data miners and optimizers then we can (a)~better understand user goals to (b)~produce results that are more relevant to our clients.

To understand this point, we first note that modern data miners run so quickly since they are highly optimized to achieve a single goal (e.g. minimize class  entropy or variance). But there are many situations where the business users have {\em multiple} competing goals; e.g. deliver {\em more} functionality,
in {\em less} time, with {\em fewer} bugs. 
A standard data miner (e.g. CART) can be kludged to handle multiple goals reasoning, as follows: compute the class attribute via some {\em aggregation function} that uses some ``magic weights'' $\beta$, e.g., $\mathit{class\;\textunderscore value}= \beta_1\times\mathit{goal1} + \beta_2\times\mathit{goal2} + ...$
%\[
%\mathit{class\;\textunderscore value}= \beta_1\times\mathit{goal1} + \beta_2\times\mathit{goal2} + ...
%\]
But using an aggregate function for the class variable is a kludge, for three reasons.
Firstly, when users change their preferences about $\beta_i$, then the whole inference must be repeated.

Secondly,
the $\beta_i$ goals may be inconsistent and conflicting. A repeated result in decision theory is that user preferences may be nontransitive~\cite{Fishburn1991} (e.g. users rank $\beta_1<\beta_2$ and $\beta_2<\beta_3$ but also $\beta_3<\beta_1$). Such nontransitivity means that a debate about how to set $\beta$ to a range of goals may never terminate.

Thirdly, rather than to restrict an inference to the whims of one user, it can be insightful to let an algorithm generate solutions across the space of possible preferences. This approach was used by Veerappa et al.~\cite{Veerappa11} when exploring the requirements of the London Ambulance system. They found that when they optimized those requirements, the result was a {\em frontier} of hundreds of solutions like that shown in \fig{veer}. Each member of that frontier is   trying to push out on all objectives (and  perhaps failing on some). Mathematicians and economists call this frontier the {\em Pareto frontier~\cite{pareto1906manuale}}. Others call it the {\em trade-off space} since it allows users to survey the range of compromises (trade-offs) that must be made when struggling to achieve multiple, possibly competing, goals.

\begin{figure} 
\centering
%\includegraphics[width=4in]{fig/clusters.png}
\rotatebox{90}{\hspace{24mm} \tiny\textsf{value}}
\includegraphics[width=2.5in,trim=20 20 0 0,clip,]{fig/clusters-fromieeexplore.png}\\
\vspace{-1.5mm}\hspace{4mm}{\tiny\textsf{cost}}
%\includegraphics[width=2in]{fig/clusters.png}
\caption{Clusters of the solution frontier. Frontier generated by reasoning over the goals (in this case, {\em minimize} cost and \emph{maximize} value). Clusters generated by reasoning over the decisions that lead to those goals. From~\cite{Veerappa11}.}\label{fig:veer}
\end{figure}

\fig{veer} is an illustrative example of how data mining can help optimizers. In that figure, the  results are grouped by a data miner (a clusterer). The decisions used to reach the centroid of each cluster are a specific example, each with demonstrably different effects. When showing these results to users, Veerappa et al. can say (e.g.) ``given all that you've told us, there a less than a dozen kinds of solutions to your problem''. Note the style of this dialogue: 
\bi
\item
Step\#1: Optimize: here are the possible decisions;
\item
Step\#2: Data mine: here is a summary of those decisions;
\item Step\#3: Business users need only debate the options in the summary.
\ei

% For one example where researchers explored
% decision neighborhoods, consider the DDP and STAR
% work of  Feather and Menzies~\cite{100feather2002converging,Menzies:2007}.
% In his initial work on DDP,
% Feather used simulated annealing and genetic algorithms  to explore software requirements models at the Jet Propulsion Lab. Those requirements were represented as a large directed many-to-many mapping representing (a)~goals for the mission software; (b)~the risks to those goals; and (c)~the mitigations that could reduce that risk. Given that graph, the optimization problem was to find the least cost combination of mitigations that retired the most risks that, hence, enabled the greatest number of mission goals.  
% In that domain, simulated annealing and genetic algorithms  suffered from overfitting~\cite{100feather2002converging}. Specifically, those algorithms  made categorical decisions about whether or not to apply all mitigations. This meant that business users had to commit to decisions about all aspects of the project.

\begin{wrapfigure}{r}{2.8in}
\small
After (say) 10,000 evaluations of a simulated annealer, then
there are $B=1000$ `best' solutions and $R=9000$ rest.
\bi
\item
Let $a$ be ``analyst capability''  and  let ``$a$=high''  appear 50 times in best and 90 times in rest.
\item
Let 
$u$ be ``use of software tools'' and let ``$u$=high`` appear 100 times in best and 180 times in rest.
\item Let: 
$b_{a.high}=50/1000=0.05$\newline
$r_{a.high}=90/9000=0.01$\newline
 $b_{u.high}=100/1000=0.1$ \newline
$r_{u.high}=180/9000=0.02$.
 \item
 STAR sorts ranges via $s=b^n/(b+r)$, where $n$ is a constant
 used to reward ranges with high support in ``best''. 
E.g. if  $n=2$ then
  $s_{c.high}=0.042$ and $s_{u.high}=0.083$.
  \item
  Hence, STAR would report that high use of software tools  is more important than 
  high analyst capability.
  \ei
  \caption{  STAR   Bayesian contrast ranking procedure~\cite{Menzies:2007} uses
  $b^n/(b+r)$ as defined in this example.}\label{srank}
\end{wrapfigure} 

Another approach to understanding trade-off space is contrast-rule generation
as done by (e.g.) Menzies et al.'s STAR algorithm~\cite{Menzies:2007}, where 
STAR monitored optimizers exploring software engineering process models. 
STAR divided those results into a 10\% ``best'' set and a 90\% ``rest'' set. A Bayesian contrast set procedure was then applied to rank all $N$ decisions in descending order (best to worst). STAR then re-ran the optimizer $i\in N$ times, each time pre-asserting the first $i$-the ranges.

The result was a graph showing the effects of taking the first best decision, the first two best decisions, and so on. In this way, STAR would report to users a succinct rule set advising them what they can do if they are willing to change just one thing, just two things, etc~\cite{Menzies:2007}.

Before ending this section, we stress the following point: 
{\em it can be very simple to add a data miner to an optimizer}.
For example:
\bi
\item
STAR's contrast set procedure is shown in Figure~\ref{srank}. Given discretized attribute ranges, the procedure is around 30 lines of code (in Python).  
\item
Recall from the above that Majumder et al. speed up their optimzier by 500 to 900 times, just by prepending a k-means clusterer to an existing optimzation process. 
\ei

==> old/claim5.tex <==
\section{Claim4: Data mining without optimization is not recommended.}
\label{sec:claim5}
 

 
There are many reports in the empirical  SE literature
where the results of a data miner are used to defend claims such as: 
\bi
\item
{\em ``In this domain, the most important concepts are X.''}
For example, Barua et al.~\cite{Barua2012WhatAD} used  text mining   called  to conclude
what topics are most discussed at Stack Overflow.
\item
{\em ``In this domain, learnerX is better than learnerY
for building models.''} For example, Lessmann et al.~\cite{lessmann8} reported that the CART decision tree
performs much worse than random forests for
defect prediction.
\ei
All the above results were generated using
the default values  for CART, random forests and a particular text mining algorithm. We note that these conclusions are now questionable given that tuned learners produce very different results to untuned learners.
For example:
\bi
\item Claims like {\em ``In this domain, the most important concepts are X''} can be 
changed by applying an optimizer to a data miner. For example,
Tables 3 and 8  of~\cite{57agrawal2018wrong}
show what was found before/after tuned
text miners were applied to Stack Overflow data. In 
many cases, the pre-tuned topics just disappeared after tuning.  Also,
in defense of the tuned results, we note that, in ``order effects experiments'', 
the pre-tuned topics were far more ``unstable''
than the tuned topics\footnote{In ``order effects experiments'', the training data is  re-arranged at random  before running the learner again. In such experiments,
a result is ``unstable''
if the learned model changes just by re-ordering the training data.}.
\item Claims like {\em  ``In this domain, learnerX is better than learnerY
for building models''} can be changed  by tuning.
One example Fu et al. reversed some of the Lessmann et al. conclusions
by showing that  tuned CART  performs much better than random forest~\cite{35fu2016}.
For another example, recall \fig{tanit} where, before/after tuning the C5.0 algorithm was the
worst/best learner (respectively).
\ei

\begin{figure}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{rlr|rlr}
\multicolumn{3}{c}{Before Tuning} & \multicolumn{3}{c}{After Tuning} \\ \hline
 features & ~ & value & features & ~ & value \\\hline
rfc & \textcolor{black}{\rule{26mm}{2mm}}  &  26 & rfc & \textcolor{black}{\rule{64mm}{2mm}}  &  64 \\
avg\_cc & \textcolor{black}{\rule{9mm}{2mm}}  &  9 & moa & \textcolor{black}{\rule{10mm}{2mm}}  &  10 \\
amc & \textcolor{black}{\rule{8mm}{2mm}}  &  8 & avg\_cc & \textcolor{black}{\rule{8mm}{2mm}}  &  8 \\
lcom3 & \textcolor{black}{\rule{7mm}{2mm}}  &  7 & dam & \textcolor{black}{\rule{7mm}{2mm}}  &  7 \\
cam & \textcolor{black}{\rule{7mm}{2mm}}  &  7 & loc & \textcolor{black}{\rule{6mm}{2mm}}  &  6 \\
loc & \textcolor{black}{\rule{6mm}{2mm}}  &  6 & mfa & \textcolor{black}{\rule{2mm}{2mm}}  &  2 \\
cbo & \textcolor{black}{\rule{5mm}{2mm}}  &  5 & cam & \textcolor{black}{\rule{2mm}{2mm}}  &  2 \\
ce & \textcolor{black}{\rule{5mm}{2mm}}  &  5 & npm & \textcolor{black}{\rule{1mm}{2mm}}  &  1 \\
npm & \textcolor{black}{\rule{5mm}{2mm}}  &  5 & amc & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
moa & \textcolor{black}{\rule{4mm}{2mm}}  &  4 & ca & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
dam & \textcolor{black}{\rule{4mm}{2mm}}  &  4 & cbm & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
mfa & \textcolor{black}{\rule{3mm}{2mm}}  &  3 & cbo & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
ca & \textcolor{black}{\rule{3mm}{2mm}}  &  3 & ce & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
cbm & \textcolor{black}{\rule{2mm}{2mm}}  &  2 & dit & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
wmc & \textcolor{black}{\rule{2mm}{2mm}}  &  2 & ic & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
lcom & \textcolor{black}{\rule{2mm}{2mm}}  &  2 & lcom & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
max\_cc & \textcolor{black}{\rule{1mm}{2mm}}  &  1 & lcom3 & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
dit & \textcolor{black}{\rule{1mm}{2mm}}  &  1 & max\_cc & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
ic & \textcolor{black}{\rule{0mm}{2mm}}  & 0 & noc & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\
noc & \textcolor{black}{\rule{0mm}{2mm}}  & 0 & wmc & \textcolor{black}{\rule{0mm}{2mm}}  & 0 \\\hline
\end{tabular}
}
\end{center}
\caption{Features importance shown for decision tree before and after tuning on jEdit defect prediction where it is optimized for {\em minimizing} distance to ``utopia'' (where ``utopia''
is the point recall=1, false alarms=0).}
\label{fig:feature_importance}
\end{figure}

For a small example of this effect
(that optimizing a data miner leads to
different results), see
Figure~\ref{fig:feature_importance}. This figure
ranks the importance of different static code features in
a defect prediction decision tree.
Here ``importance'' is computed as the (normalized) total reduction of the Gini index for a feature\footnote{The Gini index measures class diversity after a set of examples is divided by some criteria -- in this case,
the values of an attribute.}.
In this case, tuning significantly improved the performance of the learner (by 16\%, measured in terms of the ``utopia'' index\footnote{The distance to of a predictor's performance to the   ``utopia''
  point of recall=1, false alarms=0.}).
After tuning:

\bi
\item
Features that seemed irrelevant   (before tuning) are found to be very important
(after tuning); e.g. moa, dam.
\item
Many features received much lower ranking (e.g. amc, lcom3, cbo).
\ei
Overall, the number of ``interesting'' features that we might choose to report as ``conclusions'' from this study is greatly reduced. 
The important point here is that, in domains where data miners can be optimized very quickly,
then it would take just a few minutes to hours
to refine and improve untuned results.
In such domains, we not do recommend
 data mining without optimization.


% \begin{figure}[!t]
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \centering
%     \includegraphics[width=.95\linewidth]{./fig/untuned.png}
%         {\bf Figure~\ref{fig:feature}a:} Feature Importance with default parameters.
%     \end{minipage}~~%
%     \begin{minipage}{.49\textwidth}
%     \centering
%         \includegraphics[width=.95\linewidth]{./fig/tuned.png}
%         {\bf Figure~\ref{fig:feature}b:} Feature Importance with tuned parameters.
%     \end{minipage}
%     \caption{Feature importance shown for decision tree before and after tuning on Jedit defect prediction data where it is optimized for D2h.}
%     \label{fig:feature}
% \end{figure}


==> old/claim6.tex <==
\section{Claim5: It is insightful to explore combinations of data mining and optimization}\label{sec:claim6}

This paper is making a ``carrot and stick''
argument. The ``stick'' was presented in the last section where it was argued that there was much to lose by not using optimizers and learners in tandem.
But what is the  ``carrot''? That is, what is to be gained by combining data miners with optimizers? 
\bi
\item
The last few sections have argued that {\IT} enables
faster hyperparameter optimization which, in turn, leads to better predictions. 
\item Also, when optimization problems
are  impractically slow to solve,
it is possible to use data mining to find simpler sub-problems that can be solved faster. 
\item
Further, the rest of this section argues that {\IT} enables (a)~better
reasoning about user goals and (b)~address the problem of ``brittle'' solutions.
\ei
The following examples  are hardly definitive and
final results. Clearly, there are  many alternative methods to achieve the results
reported below.
Hence,
we suggest that the reader views the following   as motivational initial results that require much follow-up.

% Also, one sideeffect of the following examples is the generation
% of tiny model sIn the $21^{st}$ century, much of what we see and do in the world is mediated by algorithms that (e.g.) filter our news feeds or decide if we can receive certain insurance options.  
% % Hence, there is an increasing   demand for   auditable algorithms~\cite{hempel18}. 

\subsection{Enhanced Reasoning About Goals}


% \subsection{Auditable Algorithms}
% In the $21^{st}$ century, much of what we see and do in the world is mediated by algorithms that (e.g.) filter our news feeds or decide if we can receive certain insurance options.  
% Hence, there is an increasing   demand for   auditable algorithms~\cite{hempel18}. 

% The above two examples offer some intere

% data mining can teachin optimizers and explanation seed and scalabilitiy

% optimizers can each data miners about optimization


% XXX e.g. in multiple objectives, useful for data mining

% XXX e.g. data mining lets us explain optimizers. Optimizers are usually point solutions saying ``if you do exactly this then you will get that''. As Harman points out, this kind of reasoning is brittle since it does not say how small changes to {\em this} can affect the outcome.
% (harman's quote here).

% XXXdata miners are faster

% XXX the big one: deep learning. some preliminary results in that are (suvodeep) but clearly more is needed


% using data mining to do very fast landscape mining with DM.


% explanation, generationalization ddm ->optimization

% tuning, new goals popt -< dm

% inform the cycle (e.g. the susan partington work; e.g the re02 work)

% A \IT system is like agents e.g. in active learning
% leaning over our shoulders that advise “ask this question next” [?,?] or “ignore that problem, it is not relevant to your goals” [?]. Further , those agents can guide us to produce(e.g.) very succinct models that most reflect the concerns of users [?].

% stability. worried that conclusions go away just because you make some change to your optimizer that it tweaking your hyperparamters? LDADE!


==> old/replies.tex <==
 \pagenumbering{roman}
\setcounter{page}{1}

\newenvironment{com}{\color{blue}\begin{itshape}}{\end{itshape}\vspace{1ex}}
\section*{Response to Reviewers}

We are most grateful to the Associate Editor and the anonymous reviewers for their constructive comments, which have helped to improve the quality of this paper significantly. In this response, the reviewers' comments were enumerated and are cited in blue italic, followed by our responses. We have also highlighted our modifications in the manuscript file using red to facilitate the editor's checking of our revisions. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Associate Editor}
\label{sec:AE}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{com}
Based on the 3 reviews (2 * major revision, 1 reject), we recommended a ``Major Revision.''

Special attention should be paid to:
\begin{itemize}
    \item Clarify how the paper evaluates the 1st claim
    \item Discuss the SE community can make use of the 1st, 2nd, and 3rd claims
    \item Tone down the 4th claim and/or add more data to support the claim
\end{itemize}

Please provide a detailed *point-by-point* response letter to identify how the reviewers' feedback has been addressed in the revision.
\end{com}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 1}
\label{sec:Reviewer1}
\renewcommand*{\theenumi}{1.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}
\item \begin{com}This paper argues that there should be a new area of research in empirical software engineering research and practice where data mining and optimization should be combined and should assist each other for better and scalable outcome. The authors made four claims, (1) Optimization and data mining are very similar, (2) Optimizers can greatly improve data singers, (3) Data miners can greatly improve optimization and (4) Data mining without optimization should be deprecated.
\end{com}

\item \begin{com}
The paper reads well and the claims were made based on the survey data they collected. I also fully agree with the first three claims. However, I have a concern on the fourth claim, Data mining without optimization should be deprecated. I don't  agree with this statement. MSR community has been exploring lots of novel ideas and insights from the Data without applying search based SE  or optimization if you say. These studies have been useful as we see as a community. I agree that exploiting optimization would make them only better. However, I don't really agree that they should be deprecated.
\end{com}

Thank for you that comment. You are quite correct: we overstated claim4. In this draft we have made numerous changes that  
moves   ``deprecated'' to ``not recommended''. Our text is now less ardent and now politely suggests
to researchers that they might want to consider adding an optimization step to their work.
Thank you for that clarification. 



Markus: "deprecated" is still used on pages 2/16/17. Do we replace ``Data mining without optimization should be deprecated'' with ``Data mining without optimization should be recommended''... I mean ``Data mining with optimization is recommended''? If so, then this sounds like Claim2 ``Optimizers can grearly improve data miners''. Claim4 forms the core of the paper, IMHO. In search for a better formulation of Claim2, after checking \url{https://www.thesaurus.com/browse/deprecate}:
\begin{itemize}
    \item ``Data mining and optimization should go hand-in-hand from now on.''
    \item ``We disapprove of the use of data-mining without optimization, and vice versa.''
    \item ``We foresee a prosperous future for combinations of data mining and optimization.''
    \item ...
\end{itemize}

%PS1: reviewer 1 hates claim 4, and reviewer 3 loves it :-)


\item \begin{com}
While I was not fully happy with their conference submission, I even liked that one better than this version since that version provided some resources in these two areas. I was particularly happy that someone new in the area could be benefited from such resources. However, this extended version does not really add much. What is says we already know (the first three claims). Their support of data on those claims do not add much. As I noted, I could select another subset of data and draw some completely opposite claims. And for the fourth claim, I don't think they can even claim that with such a minimal set of data. Did they review the complete body of knowledge in empirical software engineering? 
\end{com}

Thank you for your comment. We have changed this draft to stress
the importance of this ``dual apporach'' as follows:
\bi
\item
leandro no more bias here. and added to text somehow
\item 
The  SE communities
exploring optimisation and data mining usually meet at seperate conferences and do not inter-mingle (see the SSBSE and MSR communities).
\item 
More things happen when you combine these methods than when you treat them separately. If optimizers are added
to data miners then data miners need not be rigid only-seeking-one-goal algorithms (this is useful since business problems are multi-dimensional
in nature where users want to satisfy many competing goals). 
\item
Also,  if data miners are added to optimizers then optimizers can run much faster since they need not explore the whole space, just the critical bits found by the data miner. 
\item
Lastly,  data miners lets us generalize across the output of the optimizers (so instead of the optimizer reporting 1000 candidate solutions, the data miner can report what is true across all this solutions, as well as sub-regions where those solutions are interestingly  different). 
\ei


\item \begin{com}
I would consider this paper if the authors tone down their claims and/or add more data to support the claims while they would need to judge papers of diverse areas in empirical software engineerings. 
\end{com}

Please see above.

\item \begin{com}
The readability of the paper is also not very good. Most often the paper looks dense or busy. Even if someone just reads the abstract, it is hard to understand what do they really mean. I suggest that the authors do a careful job in writing and presentation of the findings. 
\end{com}

That you for that comment.
Your review has  revealed that we have NOT appropriately
stressed the importance of our new methods. Nor did we frame our
final conclusions appropriately. We have made those changes in this
draft (see our above comments). 


\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 2}
\label{sec:Reviewer2}
\renewcommand*{\theenumi}{2.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}

\item \begin{com}\# Summary: Data mining and optimization are very similar

SE works should engage in optimization before publication.
OPtimization of data-mining and optimization of parameters. Default
parameters and no attempt to tease out proper performance of a learner
should be avoided when one tries to make claims: Learner X doesn't
work for SE problem Y.
The authors describe methods of optimization and data mining, show
their relationship, and the need for optimization in numerous avenues
including hyper-parameter tuning. This is important because it melds 2
SE communities closer together with some helpful tips.
\end{com}

Thank for that comment. 

\item \begin{com}
\# Recommendation: Major Revision

Why? I feel a lot of the discussion is lacking and the paper isn't
clear enough for the average SE grad student to understand.
\end{com}

we need someway to address this
https://github.com/ai-se/dataDriveSBSE/issues/42

\item \begin{com}
\# Is the work different from the MSR paper?

As a prior reviewer for the MSR paper this work is significantly
different.
\end{com}

\item \begin{com}
\# Fixes needed

Can you address the issue of locally optimized versus say general
performance? Should all our results be optimized or should we report
the range of results?
\end{com}

This is an excellent point since it raises the issues of the
uses cases of a model. As described in XXX, we can use your criteria
to better motivate this work, and give an introductory example
to the  whole DUO process.



\item \begin{com}
Page 2 line 31 needed by [100] please make sure that citations are
nouns and not parentheticals, it makes it hard to read. e.g. So\&So et
al.[100] is better than [100] on its own.
\end{com}

Fixed. Thank you for the comment.

\item \begin{com}
Page 15 Figure 4 is an unreadable screenshot. Please steal that image
better and cite the authors names DIRECTLY in the reference.
\end{com}


Fixed. Thank you for the comment.

\item \begin{com}
Why is the algorithm a figure. Figure 5. Why is it inline?
It could be just text. This is weird. Please fix.
\end{com}


XXX volunteer please

\item \begin{com}
\# Clarity:

The biggest barrier the original paper suffered from and that this
paper faces is clarity. 2 communities are being involved so examples
and clarifications across fields would be of value.

* Define data-mining up front. You're using a subset of MSR work as
  data-mining and it is not exactly what the boundaries of data mining
  are.
\end{com}

LEANDRO: I think your text for claim1, while certainly rigorous, runs the risk of being too arcane.

can you make another stab at  the claim1 text, this time offering gentle intros to data mining and optimization

https://github.com/ai-se/dataDriveSBSE/issues/46

\item \begin{com}
* URL in table 2 should be an actual figure: \\
  \url{https://raw.githubusercontent.com/txt/ase16/master/img/rankvscountvsdepth.png}
\end{com}

Thanks for your comment, we have changed it to text.

\item \begin{com}
* Algorithm (1) the optimization needs to be clarified, the use of g'
  and g'' when g and h were already availabled.
  Give g' and g'' names. Not just purposes.
\end{com}

LEANDRO: is this for you

\item \begin{com}
* Furthermore you define CONVEX optimization. This is SE, there's no
  guarantees of convexity in many problems. So why limit the
  definition to convex optimization? Many forms of Heuristic search are
  heavily used in the rest of your paper and do not need convex optimization.
  Line 10 on page 5 referring to convex optimization should be more specific.
\end{com}

LEANDRO: is this for you? can u relax a little on the standard characterizations? convex etc

\item \begin{com}
* You are writing to readers of many fields. Using the term ``samplers"
  for various forms of heuristic search either needs a clarification
  point whereby you name some individuals, or you use terminology from
  a particular field---such as search.
\end{com}

need a list of key terms in the paper, with definitions

XXX volunteer please

Markus: or: what is a sampler? Essentially, this word is used only on page 13 (with a brief reference on page 18). Can we get around the term "sampling/sampler"? Even local search "samples", and random search does this, too. I'm at a loss here.

\item \begin{com}
\# Missing discussion

- Evaluation measures that are SE relevant. THings like cost and time
  limits. We need to discuss that optimization should not be for
  IR/ML performance measures but task performance (like cost).
\end{com}

XXX volunteer please. leandro or markus

Markus: I do not understand what the reviewer is after. Can someone please point me at a page? Is it time to add fig4eval.tex again?

\item \begin{com}
\# A general gripe

I felt like other search, less optimization based, cross-overs were being
 ignored in favor of DUO. A lot of information and suggestions about priors
 mined from existing software was kind of glossed over. There were 
mentions in the paper but if you have time can you try to prop up the mining
 leg as priors are often valuable.
 \end{com}
\end{enumerate}

i think we can dodge this one. unless someone can volunteer something?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Reviewer 3}
\label{sec:Reviewer3}
\renewcommand*{\theenumi}{3.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}

\item \begin{com}Summary: The paper is about DUO: datamining using/used by optimizers. The authors argue that optimization and data mining go hand-in-hand and that every time some machine learning lago is used, there should be optimization. They have 4 claims in the paper. Some are supported by literature and one is argued logically. They also carry out a literature survey on the subject matter.
\end{com}

\item \begin{com}
Review:

I agree with the suthors that optimization must happen whenever ML algos/models are used in SE. Additionally, I like the literature review done by the authors. Table 1 and claim 4 (and partly 3) are very cool contributions.
\end{com}

Thank you for those kind words.

\item \begin{com}

However, I find a considerable portion of this work highly misplaced. Why is this paper at EMSE? What is the value of claim 1 for SE folks (practitioners and researchers)? I can see how claim 4 is useful. Letting us know that as researchers we should not be using ML models without optimizing for hyperparamenters. Let me present issues claim by claim.
\end{com}


Initial thoughts: regarding claim 1 -- can we argue that claim 1 is the foundation based upon which the other claims were built? One needs to know claim 1 to be able to contribute with claims 2-3, and perhaps also claim 4. 

To me, claim 1 is also the minimum knowledge that a software engineer should have before applying DUO. They should not be applying something that they have no idea what it is, and claim 1 is necessary to enable software engineers to have at least some knowledge of what DUO is. I wonder if the reviewer could also accept this argument. And, our paper explains it concisely, rather than requiring software engineers to read a whole book on optimization and another one on data mining before being able to infer that themselves.

Regarding EMSE, the paper is about the contributions that DUO can make to software engineering, and is based on a systematic literature review in the context of software engineering. Perhaps if we further improve our discussion on how our claims can benefit the software engineering community, we can address this comment?

\item \begin{com}

Claim 1: Optimization and data mining are very similar. Ask any core ML person and they would say all of it is nothing but optimization. In fact all ML theory people are essentially mathematicians who do optimization. Now I am not an ML theory person. And neither are any of the readers or reviewers of EMSE journal. So my questions are:

a) How can we evaluate the claim? \\
b) Is this a new finding? Have ML theory people not done this? Why present in a SE journal? \\
c) What is the claims connection to SE? No motivation at all here for the required audience. 
\end{com}

Leandro: i think we can get out of this one with a gentler
 claim1 comment. Perhaps you'd consider using fig2 from
 
\url{https://www.researchgate.net/publication/220343868_ROC_n_Rule_LearningTowards_a_Better_Understanding_of_Covering_Algorithms } 

and the neural net minimzation example from
\url{https://www.willamette.edu/~gorr/classes/cs449/momrate.html}


Comment (not necessarily to be discussed in our response): ``Ask any core ML person and they would say all of it is nothing but optimization.'' Actually, this is not true. Optimisation people tend to think that ML is all about optimisation. Machine learning people tend not to agree with that, due to the need for generalization. The use of optimization is just the means to solve ML problems, given that we do not have knowledge about the true underlying distribution of the problem. The theory of ML is based on the need for generalization, which is not necessarily the case for optimization. So, optimization and ML are similar in terms of the solution to the problem, but they are not necessarily similar in terms of the problem that we are trying to tackle. Of course, when we start discussing the fact that the fitness functions of our optimization problems may be uncertain, then generalization also becomes important in optimization problems, which is something that the ML people don't usually realize. We need to double check if anyone has written a discussion about this in the literature.

Initial thoughts: see previous reviewer comment.


\item \begin{com}

Claim 2: Optimizers can improve data mining. I like the fact that SE research is used to support this claim. I would like to know if there are any findings that are specific to SE data? I do learn that there are quite a few papers that do this. So what? What ways are data mining SE data being improved by optimizers. 
\end{com}

TIMM: handle this one. Amrit's new results

\item \begin{com}

Claim 3: Data miners improve optimization. Similar to claim 1, is this a new finding? What is novel about this? Why should it be in SE journal?
\end{com}

Timm: because AI software is software etc etc.   dave bibkey. beawre other people's AI.

\item \begin{com}

Claim 4: I really like this claim. There is value for an SE audience. The two examples are excellent. 
\end{com}

Thank you for your kind words.

Note that some of your above issues, on the the other claims,
are deliberate design choices on our part. We think our message is very radical so this whole paper is an exercise in gently leading
newcomers into this arena (particularly claim4). Now these reviews
have shown us that we need, sometimes, to hurry up a little and drop and 
more key points along the way-- which is feedback we have used in this draft.

\item \begin{com}

Research direction: The first one is relevant to SE. The 2nd one (with 4 directions) are not SE related. I am not sure how or why these directions came from the result of this paper. Are these an exhaustive list? 
\end{com}

As you have observed, this is hardly an exhaustive list. But, with respect,
we disagree that they are not SE related. There are many things that seem distant to SE but research has shown are core issues (category theory, context free grammars, non-linear dyncamics). Timm XXX more valium here please.

\item \begin{com}

Overall, I think some parts of this paper can be taken and a good IEEE SW paper maybe written. But otherwise, there is not much research here for a paper in EMSE. This is just not the right audience to evaluate if the findings are novel, the proofs are correct (or if there are better proofs), and the results useful. 
\end{com}

TImm: reviwer valium here please

\item \begin{com}

Smaller issues:
1) Table 1 showing more interest in 2018 in this topic might be a factor of the search space. All papers in 2017-18 were used, while only papers with a certain amount citations were considered from the past. Lose either the citations condition or the year condition. 
\end{com}

Timm: push back on this one

Initial thoughts: I agree, and I had actually raised this issue myself before we submitted our paper. We can't really deal with this issue apart from discussing the fact that indeed there is a risk that this perceived increase in the attention is due to the search space.
\end{enumerate}


 


==> old/theend.tex <==
\section{Research Direction}

One way to assess any proposed framework such as {\IT} is as follows:
is it sufficient to guide the on-going work of a large community of researchers? As argued in this section, {\IT} scores very well on this criterion.

Firstly, given  that {\em data mining without optimization should be deprecated}, it is time to revisit and recheck every prior software analytics result based on untuned data miners. This will be a very large task that could consume the time of hundreds of graduate students for at least a decade.

Secondly, given that {\em  data miners can greatly improve optimizers}, there are many research directions:
\bi
\item  {\em Better explanation and comprehension tools for AI systems:} Use the data miners to summarize complex optimizer output in order to convert opaque inference into something comprehensible. Some methods for that were seen above in \fig{veer} and Figure~\ref{srank} but they are just two early prototypes. Adding comprehension tools to AI systems that use optimization
is a fertile ground for much future research. For
a discussion on criteria to assess comprehensibility in software
analytics, see~\cite{Mori2018,Chen2018ApplicationsOP}.
\item {\em Auditable AI:} There is much recent interest in allowing humans to query AI systems for their biases and, where appropriate, to adjust them. Sampling tools like those of Chen and Nair et al.~\cite{31chen2018,89chen2018sampling,90nair2018finding}  offer  functionality that might be particularly suited for  that task. Recall that these tools optimized their models using just a few dozen examples -- which is a number small enough to enable human inspection. Perhaps we could build human-in-the-loop systems where humans watch the samplers' explored options -- in the field of optimization, the concepts of interactive optimization, dynamic optimization, and the multi-objective encoding of user preferences are well-established.
At the very least, this might allow humans to understand the reasoning.
And at the very most, these kinds of tools might allow humans to ``reach  in'' and better guide the reasoning.
\item {\em Faster Deep Learning:}
One open and pressing issue in software analytics is the tuning of deep learning networks. 
Right now, deep learning training is so slow that it is common practice to download pre-tuned networks. This means that  deep learning for software analytics may be prone to all the problems we discussed in claims 2 and 4. We gave some ideas here on how data mining can divide up and simplify the deep learning training problem (but, at this time, no definitive results).
\item
{\em Avoiding Hyper-hyperparameter Optimization:} While hyperparameter optimization is useful, it should be noted that the default parameters of hyperoptimizers may themselves need optimizing by other optimizers. This is a problem since if hyperparameter optimization is slow, then hyper-hyperparameter optimization would be even slower. 
So how can we avoid  hyper-hyperparameter optimization?
\bi
\item
One possible approach is {\em transfer learning}. Typically when something is tuned, we do so because it will be run multiple times. So instead of search
{\em taula rasa} for good tunings, perhaps it is possible to partially combine parts of
old solutions to speed up the search for good hyperparameter values~\cite{Nair2018TransferLW}.   
\item
An analogous approach is to   select from a portfolio of algorithms. This typically involves the training of machine learning models on performance data of algorithms in combination with instances given as feature data. In software engineering, this has been recently used as for the Software Project Scheduling Problem \cite{Shen2018,wu2016}. The field of per-instance configuration has received much attention recently, and we refer the interested reader to a recent updated survey article~\cite{kotthoff2016survey}. 
\item
Another approach, is to find shortcuts around the  optimization process. For recent work on that, which we would characterize as highly speculative, see~\cite{fu2018building}.
\ei
\ei
Thirdly, given that  {\em optimizers can greatly improve data miners}, it is time to apply hyperparameter optimization to more data mining tasks within software analytics. As shown by this paper, such an application can lead to dramatically better predictors.
Moreover, given that multi-objective perspective that can be given by optimizers, we can use optimizers to enable data mining to explore multiple objectives. For example:
\bi
\item
For software analytics, we could try to learn data miners that find highest priority bugs 
after the {\em fewest} tests, found in the {\em smallest} methods in code that is {\em most familiar} to the current human inspector.   Such a data miner would return the bugs 
that are most important and easiest to fix (thus reducing issue resolution time for important issues).
\item
For project management,
when crowd sourcing large software projects, we could allocate tasks to programmers in order to {\em minimize} development time while {\em maximizing} work assignments to programmers that have   most familiarity with that area of the code.
\item
For refereeing new research results in SE, the tools described here could  assign reviewers to new results in order to {\em minimize} the number of reviews per reviewer while {\em maximizing} the number of reviewers who work in the domain of that paper.
\ei

\noindent We could also extend SE to make it about using DUO for providing software engineering support for artificial intelligence
systems. For example, using the optimization discussed above, 
Weise et al.~\cite{Weise2018AnIG} have run over 157 million experiments on over 200 instances of two classical AI combinatorial problems. They found that the naive configuration is a good baseline approach, but with effort it was possible to outperform it. Friedrich et al.~\cite{Friedrich2018EscapingLarge} who studied a
particular family of heuristic hill-climbers problems.
Their empirical optimization results sparked extensive theoretical investigations (i.e., proper computational complexity analyses) that showed that the new configuration is provably faster than what has been state-of-the-art. These can be seen as examples of software engineering to find better configurations. Other work in this area includes
Neshat et al.~\cite{Neshat2018waveenergy} who studied wave energy equations. 
Their optimization results were translated into well-performing algorithms for large problems.  This can be seen as software engineering to improve algorithms' performance.



Lastly, given  {\em that data mining and optimization is
essentially the same thing}, it is time to explore engineering principles for creating unified data mining/optimizer toolkits. We already have one exemplar of such a next-generation toolkit: see \url{www.automl.org} for the work on AutoML and its connections to Weka and scikit-learn. That said, this research area  is wide open for experimentation. For two reasons, we would encourage researchers to ``roll their own''
{\IT} implementations before automatically turning to tools like AutoML:
\bi
\item Some initial results suggest it may not be enough to just use AutoML~\cite{Tu2018IsOH} (in summary, given $N$ hyperparameter optimizers, AutoML was ``best'' for a miniority of goals and datasets). 
\item In terms of training ourselves on how easy it is to combine optimizers and data miners, there is no substitute for ``rolling your own'' implementation (at least once, then perhaps moving on to tools like AutoML).
\ei


 
  


% avoid hyper-hyper parameter optimization 
% $\rightarrow$ The tuning of algorithm tuners is extremely time-consuming. While Dang et al.~\cite{dang2017iraceconfig} recently used surrogate functions to speed up the optimizer tuning, more research is needed for the optimization of optimizers more widely applicable. 




% basis for further work by a large team 
% XXXX deep learning ---  Whether or not we should use it will depend on the problem and on whether or not the researchers/customers are happy with a ``magical black box''. 
% The production use of deep learning in speech recognition and self-driving cars shows that the black box characteristic is not necessarily a problem.
% Technically, an alternative for some problems is the aforementioned genetic programming, where graphs are evolved that can represent human-readable formulae and programs. There is, however, little hardware support for and education about genetic programming.

% education about {\IT}
% at conferences: tutorial speakers to be bold and to reach out to other events 
% in higher education: add a lecture or two into a course (Markus will add a lecture and exercise on automated algorithm configuration to his SBSE'19 course)
% in research: do a literature review, and don't be afraid to reach out (getting all warm and fuzzy)

%  We need better integration of data miners and optimizers in the current tool kits. Auto-weka is a good start, similarly auto-sklearn is a automated approach to model building based on sklearn (i.e., it tries out lots of different techniques and does the tuning of the techniques along the way). Before anyone jumps right into this and sees these integrated packages as one-size-fits-all solutions, a word of caution. As powerful as they are, it is also easy to set them up in a sub-optimal way that does not let them make use of all their algorithmic power. We highly recommend to start with a basic an manually setup approach first, to get a feel for the behavior and the involved learning times. 

% Speaking of which: in new papers, it would be great to see fewer comparisons of the style ``new vs really old'' and more comparisons like ``new vs recent approach'', given the general availability of code and tools.%talking against a wall, probably

% Auditable algorithms. given the  $O(2{\log}(N))$ results seen above, can we get humans in the loop to supervise, audit, approve, adjust conclusions of these {\IT} systems.

% Education



% % We recommend that you all talk to each other: optimizers to data miners, and vice versa. Much can be gained from combining fundamental algorithmic understanding with approaches that work in practice.




% % \section{Summary}
% % This paper has argued for 
% % combine data miners and optimizers.

% % {\em Data mining and optimization is very similar:}. That is, it is somewhat artificial to separate the two tasks. 

% % {\em Very fast runtimes:} 
% % This combination can sometimes run much faster than a standard optimizer; e.g. see the Nair, Chen et al. results.


% % {\em Overfitting avoidance:} Smaller models use fewer variables or are simpler in structure, and hence are less prone to overfitting. They are also more immune to noise in the attributes which they ignored in their model.

% % {\em Faster hyperparameter optimization:}
% % \bi
% % \item
% % The last few sections have argued that {\IT} enables
% % faster hyperparameter optimization which, in turn, leads to better predictions. 
% % \item Also, when optimization problems
% % are  impractically slow to solve,
% % it is possible to use data mining to find simpler sub-problems that can be solved faster. 
% % \item
% % Further, the rest of this section argues that {\IT} enables (a)~better
% % reasoning about user goals and (b)~address the problem of ``brittle'' solutions.
% % \ei
% % The following examples  are hardly definitive and
% % final results. Clearly, there are  many alternative methods to achieve the results
% % reported below.
% % Hence,
% % we suggest that the reader views the following   as motivational initial results that require much follow-up.



% \subsection{Comment}

 
\section{Conclusion}

For software analytics it is 
{\em possible}, {\em useful} and 
{\em necessary} to combine data mining and optimization using {\IT}. Such combination can lead to better (e.g., faster, more accurate or reliable, more interpretable, and multi-goals) analyses in empirical software engineering studies, in particular those studies that require automated tools for analysing (large quantities of) data. We support our arguments based on a literature review of applications of {\IT}.

We say it is {\em possible} to combine data mining and optimization since data mining and optimization perform essentially the same task (Section \ref{sec:claim1}). Hence, it is hardly surprising that it can be a relatively simple matter to build a unified data mining/optimizer tool. For instance:
\bi
\item Nair et al.'s approach~\cite{90nair2018finding} was just a for-loop around CART.
\item STAR~\cite{Menzies:2007} was also a very simple learner (see Figure~\ref{srank}) wrapped around a simulated annealer, then re-ran the simulated annealer after setting the first $i$-best ranges.
\item Sampling  is just a simple bi-recursive clustering algorithm (but see {\S}3.4 of~\cite{89chen2018sampling} for a discussion on some of the nuances of that process).
\item There are many mature open source data mining and optimization frameworks\footnote{E.g. in Python: scikit-learn and DEAP~\cite{scikit-learn,rainville2012deap}.
E.g. in Java: Weka and (jMetal or SMAC)~\cite{Hall:2009,Durillo2011,hutter2011sequential}.
%E.g. language agnostic: irace and SMAC~\cite{hutter2011sequential}.
}. Also, some of the data mining and optimization algorithms 
are inherently very simple to implement (e.g. naive bayes~\cite{Frank2000}, differential evolution~\cite{Storn:1997}). Hence it is easy to implement  optimizer+data miner combinations.
\ei 
As to {\em usefulness}, this paper has listed several benefits of {\IT}:
\bi
\item Data miners can speed up optimizers by dividing large problems into several  simpler and smaller ones. 
\item Also, when optimizers return many example solutions, data miners can generalize and summarize those into a very small set of exemplars (see for example \fig{veer}) or rules (see for example Figure~\ref{srank}).
\item Optimization technology lets data miners explore a much broader set of competing goals than just (e.g.) precision, recall, and false alarms. Using those goals, it is possible
to better explore an interesting range of SE problems such as 
project management, requirements engineering, design, security problems,
software quality, software configuration,  mining textual SE artifacts,
just to name a few. 
\ei
Finally, as to {\em necessary}, we assert that it is misleading to report
conclusions from an untuned learner since those conclusions can changed by tuning.
Since papers that use untuned learners can be so easily refuted, this community should be wary of publishing analytics papers that lack an optimization component.

Having made this case, we acknowledge that {\IT} would require  a paradigm shift for the software analytics community. Graduate subjects would have to be changed (to focus on different kinds of algorithms and case studies); toolkits would need to be reorganized; and journals and  conferences will have to adjust their paper selection criteria.
Looking into the future, we anticipate several years where {\IT} is explored
by a minority of software analytics researchers. That said, by 2025,
 we predict that {\IT} will be standard and required practice in software analytics.

